Online Policy Optimization for Robust MDP

Reinforcement learning (RL) has exceeded human performance in many synthetic settings such as video games and Go. However, real-world deployment of end-to-end RL models is less common, as RL models can be very sensitive to slight perturbation of the environment. The robust Markov decision process (MDP) framework -- in which the transition probabilities belong to an uncertainty set around a nominal model -- provides one way to develop robust models. While previous analysis shows RL algorithms are effective assuming access to a generative model, it remains unclear whether RL can be efficient under a more realistic online setting, which requires a careful balance between exploration and exploitation. In this work, we consider online robust MDP by interacting with an unknown nominal system. We propose a robust optimistic policy optimization algorithm that is provably efficient. To address the additional uncertainty caused by an adversarial environment, our model features a new optimistic update rule derived via Fenchel conjugates. Our analysis establishes the first regret bound for online robust MDPs.

==> defs.tex <==
% New, for this draft only
\newcommand{\Vp}{V_h^{\pi_k}}
\newcommand{\hVp}{\hat{V}_h^{\pi_k}}
\newcommand{\Vpn}{V_{h+1}^{\pi_k}}
\newcommand{\hVpn}{\hat{V}_{h+1}^{\pi_k}}
\newcommand{\Qp}{Q_h^{\pi_k}}
\newcommand{\hQp}{\hat{Q}_h^{\pi_k}}
\newcommand{\sPsa}{\sigma_{\mathcal{P}_h(s,a)}}
\newcommand{\hPsa}{\sigma_{\hat{\mathcal{P}}_h(s,a)}}
\newcommand{\sPs}{\sigma_{\mathcal{P}_h(s)}}
\newcommand{\hPs}{\sigma_{\hat{\mathcal{P}}_h(s)}}


\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mathbb{R}}}
\newcommand{\integers}{{\mathbb{ Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\prox}{\mathbf{prox}}

\newcommand{\Expect}{\mathbb{E{}}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\epi}{\mathop{\bf epi}} % epigraph
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} % domain
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\sign}{\mathop{\bf sign}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}


\newcommand{\relu}[1]{\sigma\left(#1\right)}
\newcommand{\reluder}[1]{\sigma'\left(#1\right)}
\newcommand{\act}[1]{\sigma\left(#1\right)}

\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}[section]
\newtheorem{prop}{Proposition}[section]'
\declaretheorem[name=Proposition]{proposition}
\newtheorem{asmp}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{oracle}{Oracle}[section]
\newtheorem{fact}{Fact}[section]
\newtheorem{conj}{Conjecture}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{example}{Example}[section]
\newtheorem{condition}{Condition}[section]

%RL 
\newcommand{\levels}{[H]}
\newcommand{\fclass}{\mathcal{F}}
\newcommand{\covset}{\mathcal{M}}
\newcommand{\epsstat}{\epsilon_s}
\newcommand{\epstest}{\epsilon_t}
%\newcommand{\epsreg}{\epsilon_r}
\newcommand{\deltatrain}{\delta_{tr}}
\newcommand{\deltatest}{\delta_{te}}
%\newcommand{\dist}{\mathcal{D}}
\newcommand{\gap}{\mathrm{gap}}
\newcommand{\gapmin}{\rho}
\newcommand{\algo}{\textsf{Difference Maximization $Q$-learning}}
\newcommand{\epsn}{\epsilon_N}
\newcommand{\ridge}{\lambda_{\mathrm{ridge}}}
\newcommand{\epsr}{\lambda_r}
\newcommand{\pifinal}{\hat{\pi}}
\newcommand{\true}{$\mathrm{True}$}
\newcommand{\false}{$\mathrm{False}$}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\relearn}{$NeedToReLearn$}
\newcommand{\distmdp}{\dist_{\mathrm{MDP}}}
\newcommand{\dmdp}{d_{\mathrm{MDP}}}
\newcommand{\linopt}{T}
\newcommand{\diam}{\mathrm{diam}}
\newcommand{\srl}{\textsf{RL}}
\newcommand{\gm}{\textsf{Generative Model}}
\newcommand{\kt}{\textsf{Known Transition}}
%\def\approxcorrect{\checkmark\kern-1.1ex\raisebox{.7ex}{\rotatebox[origin=c]{125}{--}}}
\def\approxcorrect{\checkmark\kern-1.1ex\raisebox{.89ex}{$\times$}}
\newcommand{\spanner}{\Lambda}

%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\let\ab\allowbreak


==> lower.tex <==
We first describe a distribution over a set of 3-states hard problem instances. Then by Yao's principle, we hos that any deterministic algorithm that performs well on my of such instances, will fail on another one. 

Consider a set of MDP with 3 states $s_0, s_1, s_2$, and a set of actions $\gA$. Without loss of generality, we set $s_0$ to be the initial state. The reward function is defined as following. On the initial state $s_0$ and $s_2$, all action will leads to a zero rewards. On state $s_1$, all action will incur a reward of 1. The transition dynamic of the MDP is defined as follow. On state $s_0$, a special action $a^\ast$ will leads to $s_1$ with probability $0.5 + \epsilon$ and to $s_2$ with probability $0.5 - \epsilon$. For all other actions, from $s_0$, will leads to either $s_1$ or $s_2$ each with probability $1/2$. States $s_1$ and $s_2$ are self-looping, in the sense that taking any actions on these two states will leads back to it self. We remark that by constructions of these MDPs, they can be reduced to a set of bandits instance where there is one unique arm that has rewards $0.5 + \epsilon$. The only difference is that the regret now scales up by $H - 1$.

With a $(s,a)$-uncertainty set of radius $\rho$ \dong{does this work with $s$-rectangular?}, the MDP that corresponds to the distributional robust value is the following. This robust MDP will instead let the special action $a^\ast$ transits $s_1$ with probability $0.5 + \epsilon - 0.5 \rho$ and to $s_2$ with probability $0.5 - \epsilon + 0.5\rho$ from $s_0$. \dong{This is so because we required the robust MDP's transition kernel to be absolutely continuous with respect to the original one. So the transition of $s_1$ and $s_2$ to themselves have to remain unchanged. } By the same deduction logic, this set of MDPs are equivalent to a set of bandits instance where there is one unique arm that has rewards $0.5 + \epsilon - 0.5\rho$. The only difference is that the regret now scales up by $H - 1$.

For an algorithm $\gM$, let $\pi$ be the policy it learnt with access to only the nominal model and $\pi^\prime$ be the policy it learnt on the robust transition. Let $V^{\pi}(s_0)$ denotes the robust value function of policy $\pi$ and let  $V^{\pi^\prime}(s_0)$ be the robust value function under policy $\pi^\prime$. There are only two kinds of policy available for $\pi$ and $\pi^\prime$. One is to choose $a \neq a^\ast$ on $s_0$, if both policy take the non-special actions, then  $V^{\pi}(s_0) = V^{\pi^\prime}(s_0) = 0$. The other kind of policy is to choose the special action $a^\ast$. In such case, we have $V^{\pi^\prime}(s_0) - V^{\pi}(s_0) = (H - 1) ( 0.5 +  \epsilon - 0.5 \rho )( \pi(a^\ast \mid s_0) - \pi^\prime(a^\ast \mid s_0)) \geq (H - 1) ( 0.5 \rho - \epsilon - 0.5)$.
%$V^{o, \pi}(s_0) - V^\pi(s_0) = 0.5 (H-1) \rho\cdot \pi(a^\ast \mid s_0) $. 
We let $V^\ast(s_0) = \max_\pi \min_{P \in \gP} V^{\pi, P}(s_0)$ to be the the optimal robust value under the robust transition kernel and $V^{o,\ast}(s_0) = \min_{P \in \gP} \max_\pi $. Note that we also have $V^\ast(s_0) - V^{o,\ast}(s_0) = 0$, as the worst case transition kernel 4
et of robust MDPs, let us pick the special action $a^\ast$ uniformly random among all actions. For an algorithm $\gM$, let $\pi$ be the policy it learnt with access to only the nominal model and $\pi^\prime$ be the policy it learnt on the robust transition. Then the regret is 
\begin{align*}
     \text{Regret}^\pi(K) 
     = \ & V^\ast(s_0) - V^{\pi}(s_0)\\
     = \ & V^\ast(s_0) - V^{\pi^\prime}(s_0) + V^{\pi^\prime}(s_0) -  V^{\pi}(s_0)\\
     = \ & V^{o, \ast}(s_0) - V^{\pi^\prime}(s_0) + V^{\pi^\prime}(s_0) - V^\pi(s_0)\\
     \geq \ & (H - 1) ( 0.5 \rho - \epsilon - 0.5) + V^{o, \ast}(s_0) - V^{\pi^\prime}(s_0) \,.
\end{align*}
By standard bandits lower bound \cite{auer2002nonstochastic} (Theorem A.2), we have the 
\begin{align*}
    V^{o, \ast}(s_0) - V^{\pi^\prime}(s_0)  = \Omega \left( HK (\epsilon - \rho) \left( 1 - (\epsilon - \rho) \sqrt{\frac{K}{A}} \right) \right) \,.
\end{align*}
For $K \geq 4$, 
\begin{align*}
    \text{Regret}(K) 
    \geq \ & K(H - 1) ( 0.5 \rho - \epsilon - 0.5) +  \Omega \left( HK (\epsilon - \rho) \left( 1 - (\epsilon - \rho) \sqrt{\frac{K}{A}} \right) \right) \\
    \geq \ & K\left( \frac{1}{\sqrt{K}} + \epsilon - \rho\right) + \Omega \left( HK (\epsilon - \rho) \left( 1 - (\epsilon - \rho) \sqrt{\frac{K}{A}} \right) \right) \,.
\end{align*}
Take $\epsilon = (1-\rho) \sqrt{\frac{A}{K}} + \rho$, then we have
\begin{align*}
    \text{Regret}(K) 
    \geq \Omega \left( \rho(1- \rho) H \sqrt{AK} \right)\,.
\end{align*}
%Notice that because $\rho \leq 1$, take $\epsilon = \rho \sqrt{\frac{A}{K}} + \rho$ we have
%\begin{align*}
%    \text{Regret}(K) = \max_{\pi} \text{Regret}^\pi(K) = \Omega(H ( 0.5 \rho - \epsilon ) + \rho H\sqrt{A K} )\,.
%\end{align*}



==> s_rect.tex <==
\begin{restatable*}[Regret under $s$-rectangular uncertainty set]{thm}{s}
\label{thm:s}
Setting $\beta = \sqrt{\frac{2 \log A}{H^2 K}}$, the regret of Algorithm is bounded by 
\begin{align*}
    \text{Regret}(K) 
    = \Tilde{O} \left( (\rho + H) SA H\sqrt{K} \right) \,.
\end{align*}
\end{restatable*}

\paragraph{Design of bonus function}
\begin{align*}
    b_h^k(s,a) = (2 \rho + 4H)\sqrt{\frac{4 S A\log(6SAH^2K^{3/2} / \delta)}{N_h^k(s,a)}} + 2 \frac{(A ( 2 + \rho) + 2)}{\exp(1/A^2)\sqrt{K}}  + \sqrt{\frac{2 \log(3SAH^2K/ \delta)}{N_h^k(s,a)}}  \,.
\end{align*}

\paragraph{Decomposition and OMD regret}
Similar to the $(s,a)$-rectangular case, we have
\begin{align*}
     \sum^K_{k=1}V_1^{\pi_\ast}(s) - \hat{V}_1^{\pi_k}(s) = \Tilde{O} \left(H^2\sqrt{K} \right)\,.
\end{align*}
{\color{blue} TODO: Need to create good events. }


\paragraph{Bounding the estimation error}
Similar to the case with $(s,a)$-rectangular uncertainty set, we have
\begin{align*}
    & (\hat{V}_1^{\pi_k} - \hat{V}_1^{\pi_k})(s) \\
    \leq \ &\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ (r(s, a) - \hat{r}(s, a)) + \left( \hPs (\hVpn)(s,a)  - \sPs(\hVpn)(s,a)\right) + b_h^k(s,a)\right]\,.
\end{align*}
Thus the key is to upper bound $\left( \hPs (\hVpn)(s,a)  - \sPs(\hVpn)(s,a)\right) $.
By the definition of $s$-rectangular set, we have
\begin{align*}
     & \sPs (\hVpn)(s,a) = \inf_{P_h \in \gP_h(s)} \sum_{s^\prime} P_h(s^\prime \mid s,a) \hVpn(s^\prime) \\
     \text{subject to } & \sum_{s^\prime, a^\prime} | P_h(s^\prime \mid s,a^\prime) - P_h^o(s^\prime \mid s,a^\prime)| \leq A\rho \,, \\
    &  \sum_{s^\prime} P_h(s^\prime \mid s,a^\prime) = 1 \,, \quad  \forall a^\prime \in \gA\\
    &  P_h(\cdot \mid s,a^\prime) >> P_h^o(s^\prime \mid s,a^\prime)\,, \quad  \forall a^\prime \in \gA\,.
\end{align*}

Define $\Tilde{P}_h(s^\prime \mid s, a) = \frac{ P_h(s^\prime \mid s,a) }{ P_h^o(s^\prime \mid s,a)}$, we can rewrite the above optimization problem as 
\begin{align*}
     &\inf_{P_h \in \gP_h(s)} \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) \hVpn(s^\prime) \\
     \text{subject to } & \sum_{s^\prime, a^\prime} | (\Tilde{P}_h(s^\prime \mid s,a^\prime) - 1| P_h^o(s^\prime \mid s,a^\prime) \leq A\rho \,, \\
    &  \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a^\prime)P_h^o(s^\prime \mid s,a^\prime) = 1 \,, \quad  \forall a^\prime \in \gA\\
    &  \Tilde{P}_h(\cdot \mid s,a^\prime) \geq 0\,, \quad  \forall a^\prime \in \gA\,.
\end{align*}
We can then obtain the Lagrangian $L(\Tilde{P}_h, \eta, \lambda)$ with $\eta = \{\eta_a\}_{a\in\gA}, \eta_a \in \mathbb{R}$, $\lambda \geq 0$.

\begin{align*}
    L(\Tilde{P}_h, \eta, \lambda) (s,a) 
    = \ & \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) \hVpn(s^\prime) + \lambda \left( \sum_{s^\prime, a^\prime} | (\Tilde{P}_h(s^\prime \mid s,a^\prime) - 1| P_h^o(s^\prime \mid s,a^\prime) - A\rho \right) \\
    & \ - \sum_{a^\prime} \eta_{a^\prime} \left( \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a^\prime)P_h^o(s^\prime \mid s,a^\prime) - 1 \right) \,.
\end{align*}

Let $f(x) = |x - 1|$, then the convex conjugate of $f$, $f^\ast(y) = \sup_{x} \limits ( \langle x, y\rangle - f(x) )$. 
Using $f^\ast$, we can rewrite the Lagrangian over as 
\begin{align*}
    & L(\Tilde{P}_h, \eta, \lambda) (s,a) \\
    = \ & - \lambda A \rho + \sum_{a^\prime} \eta_{a^\prime} + \lambda \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \left( f\left(\Tilde{P}_h(s^\prime \mid s,a^\prime) \right) - \Tilde{P}_h(s^\prime \mid s,a^\prime) \left(\frac{\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime)}{\lambda} \right)\right) \,.
\end{align*}
Thus using the convex conjugate, we can optimize over $\Tilde{P}$ and obtain
\begin{align*}
    L(\eta, \lambda) (s,a) =  - \lambda A \rho +  \sum_{a^\prime} \eta_{a^\prime} - \lambda \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) f^\ast \left( \frac{\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime)}{\lambda}\right) \,.
\end{align*}
Notice that when $x \geq 0$, $f^\ast(y)$ has value $-1$ when $y \leq -1$, $f^\ast(y)=y$ when $y \in [-1, 1]$ and $f^\ast(y) = \infty$, when $y > 1$. Let $\Tilde{\eta} = \eta + \lambda$, then using the values of $f^\ast(y)$ and the equality $\max\left\{a,b\right\} = (a - b)_{+} + b$, we can rewrite the optimization problem as
\begin{align*}
    \sup_{\lambda \geq 0, \  (\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime))_{+}\leq \lambda, \ \forall a}
    - \lambda A \rho + \sum_{a^\prime} \eta_{a^\prime} -  \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \max\left\{\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime), -\lambda\right\} \,.
\end{align*}

Let $\Tilde{\eta}_{a} = \eta_a + \lambda$, then using the identity $\max\{a, b\} = (a -b)_{+} + b$,  the problem is equivalent to
\begin{align*}
     \sup_{\lambda \geq 0, \  (\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime))_{+}\leq 2\lambda, \ \forall a^\prime,s^\prime} - \lambda A (\rho + 2) + \sum_{a^\prime} \Tilde{\eta}_{a^\prime} -  \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \left(\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} \,.
\end{align*}

Optimize over $\lambda$, we can reduce the problem into only optimizing with respect to a $A$-dimensional vector $\Tilde{\eta}$.
\begin{align*}
    \sup_{\Tilde{\eta}} \ \sum_{a^\prime} \Tilde{\eta}_{a^\prime} -  \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \left(\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} - \max_{s^\prime, a^\prime}\frac{A (\rho + 2) (\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime))_{+}}{2} \,.
\end{align*}

Define $g(\Tilde{\eta}, P_h^o)$ as 
\begin{align*}
    g(\Tilde{\eta}, P_h^o) 
    = \ &  - \sum_{a^\prime} \Tilde{\eta}_{a^\prime} +  \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \left(\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} + \max_{s^\prime, a^\prime} \frac{A (\rho + 2) (\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime))_{+}}{2} \,.
\end{align*}

First notice that $g$ is a convex function with respect to $\Tilde{\eta}$. Moreover, the infimum of $g$ can be achieved when $\Tilde{\eta}$ is a zero vector. 
Then, restricting each value in $\Tilde{\eta}$ to take values $\geq 0$, we have
\begin{align*}
    g(\Tilde{\eta}, P_h^o) 
    \geq \ & - \sum_{a^\prime} \Tilde{\eta}_{a^\prime} + \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \left(\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right) + \max_{s^\prime, a^\prime} \frac{A (\rho + 2) (\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime))_{+}}{2} \\
    \geq \ & \max_{s^\prime, a^\prime} \frac{A (\rho + 2) (\Tilde{\eta}_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime))_{+}}{2} - H \,.
\end{align*}
When $\Tilde{\eta}_{a^\prime} = 3 H + 2 \rho$, $\forall a^\prime \in \gA$, $g(\Tilde{\eta}, P_h^o) \geq  A (2 + \rho)(\rho + H) - H \geq 0$. Thus, it suffice to optimize within the interval of $\eta_{a^\prime} \in [0, 3 H + 2 \rho]$, $\forall a^\prime$. 

We can now rewrite $ \sPs (\hVpn)(s,a)  - \hPs(\hVpn)(s,a)$ as 
\begin{align*}
     \hPs (\hVpn)(s,a)  - \sPs(\hVpn)(s,a)
     = \ & \inf_{\eta_{1, a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} g(\eta_1, \hat{P}_h) - \inf_{\eta_{2, a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} g(\eta_2, P_h^o) \\
     \leq \ & \sup_{\eta_{a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} \left|g(\eta, \hat{P}_h^o) -  g(\eta, P_h^o) \right| \,.
     %= \ & \sup_{\eta_{a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime}  \left|g(\eta, \hat{P}_h^o) -  g(\eta, P_h^o) \right| \,.
\end{align*}

By Holder's inequality, we have
\begin{align*}
    &  \left|g(\eta, \hat{P}_h^o) -  g(\eta, P_h^o) \right| \\
    = \ &  \sum_{s^\prime, a^\prime} \hat{P}_h(s^\prime \mid s,a^\prime) \left(\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} - \sum_{s^\prime, a^\prime} P_h^o(s^\prime \mid s,a^\prime) \left(\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} \\
    = \ & \sum_{a^\prime} \left( \sum_{s^\prime}  \hat{P}_h(s^\prime \mid s,a^\prime) - P_h^o(s^\prime \mid s,a^\prime) \right)\left(\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} \\
    \leq \ & \sum_{a^\prime} \left\| \hat{P}_h(\cdot \mid s,a^\prime) - P_h^o(\cdot \mid s,a^\prime) \right\|_1 \left\| \left(\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} \right\|_\infty \,. 
\end{align*}

With Hoffding's inequality and the fact that we optimize within the range of $\eta_{a^\prime} \in [0, 3 H + 2 \rho]$, $\forall a^\prime$, we have the following inequality holds with probability at least $1 - \delta$,
\begin{align*}
    \sum_{a^\prime}\left\| \hat{P}_h(\cdot \mid s,a^\prime) - P_h^o(\cdot \mid s,a^\prime) \right\|_1  \left\| \left(\eta_{a^\prime} - \mathbb{I}\{a^\prime = a\} V_{h+1}^{\pi_k}(s^\prime) \right)_{+} \right\|_\infty 
    \leq \ & A(2\rho + 4H ) \sqrt{\frac{4S \log(SAH^2 K / \delta)}{N_h^k(s,a)}} \,.
\end{align*}

To bound $\sup_{\eta_{a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} | g(\eta, \hat{P}_h)  - g(\eta, P_h^o) |$ with high probability, we first create an $\epsilon$-net $N_\epsilon(\eta)$ with $g$ over $\eta\in [0, 2\rho + 2H ]$ such that
\begin{align*}
    \sup_{\eta_{a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \leq \sup_{\eta\in (\eta)} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| + 2 \epsilon \,.
\end{align*}
Taking an union bound over $N_\epsilon(\eta)$, we have 
\begin{align*}
    \sup_{\eta_{a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \leq A(2 \rho + 4H)\sqrt{\frac{4 S \log(3SAH^2K | N_\epsilon(\eta)| / \delta)}{N_h^k(s,a)}} + 2 \epsilon \,.
\end{align*}

With $\eta = \{\eta_a\}$, notice that $g$ is $(A ( 2 + \rho) + 2)$-Lipschitz. Thus we have $| N_\epsilon(\eta)| \leq \left( \frac{(A ( 2 + \rho) + 2)}{\epsilon}\right)^A$. {\color{blue} add reference here, I found it on Peter Bartlett's lecture slides.}
Thus we have
\begin{align*}
\hPs (\hVpn)(s,a)  - \sPs (\hVpn)(s,a) 
    \leq \ & \sup_{\eta_{a^\prime} \in [0, 3 H + 2 \rho], \ \forall a^\prime} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \\
    \leq \ & A(2 \rho + 4H)\sqrt{\frac{4 S A\log(3SAH^2K  (A ( 2 + \rho) + 2)/ \epsilon \delta)}{N_h^k(s,a)}} + 2 \epsilon \,.
\end{align*}

Take $\epsilon = \frac{(A ( 2 + \rho) + 2) }{2\exp(1/A^2)\sqrt{K}}$, then 
\begin{align*}
    \hPs (\hVpn)(s,a)  - \sPs (\hVpn)(s,a)
    \leq \ & (2 \rho + 4H)\sqrt{\frac{4 S A\log(6SAH^2K^{3/2} / \delta)}{N_h^k(s,a)}} + 2 \frac{(A ( 2 + \rho) + 2)}{\exp(1/A^2)\sqrt{K}} \,.
\end{align*}
By Hoeffding's inequality, we also have the following inequality holds with probability at least $1 - \delta$.
\begin{align*}
    |r(s,a) - \hat{r}(s,a)| \leq \sqrt{\frac{2 \log(3SAH^2K/ \delta)}{N_h^k(s,a)}}  \,.
\end{align*}

Thus by the design of our bonus function, we have
\begin{align*}
    \sum^K_{k=1}(\hat{V}_1^{\pi_k} - V_1^{\pi_k})(s)
    \leq \ & 2\sum^K_{k=1}\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[b_h^k(s,a) \right] \\
    = \ & \Tilde{O} \left( (\rho + H)\sqrt{SA}\right)\sum^K_{k=1}\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ \sqrt{\frac{1}{N_h^k(s,a)}}\right]  \,.
\end{align*}

By Lemma 7.5 of RL theory book {\color{blue} add reference here}, 
we have 
\begin{align*}
    \sum^K_{k=1}\sum^H_{h=1} \sqrt{\frac{1}{N_h^k(s,a)}} \leq 2 H \sqrt{SAK} \,.
\end{align*}
Combining everything, set $\delta = 1/H$, then with probability at least $1 - 2/ H$, we have
\begin{align*}
    \sum^K_{k=1}(\hat{V}_1^{\pi_k} - V_1^{\pi_k})(s) = \Tilde{O} \left( (\rho + H) SA H\sqrt{K}\right) \,.
\end{align*}

==> sa_rect.tex <==
\begin{restatable*}[Regret under $(s,a)$-rectangular uncertainty set]{thm}{sa}
\label{thm:sa}
Setting $\beta = \sqrt{\frac{2 \log A}{H^2 K}}$, the regret of Algorithm is bounded by 
\begin{align*}
    \text{Regret}(K) 
    = \Tilde{O} \left( (\rho + H) HS \sqrt{AK}\right) \,.
\end{align*}
\end{restatable*}


\paragraph{Design of bonus function}
The bonus function $b_h^k(s,a)$ is defined to be 
\begin{align*}
    b_h^k(s,a) = \sqrt{\frac{2 \log(3SAH^2K/ \delta)}{N_h^k(s,a)}} + (2 \rho + H) \sqrt{\frac{4 S \log(3SAH^2K/ \delta)}{N_h^k(s,a)}} + \frac{6 + \rho}{H\sqrt{K}}
\end{align*}

\paragraph{Decomposition and OMD regret}
We first decompose the regret as 
\begin{align*}
    \text{Regret}(K) 
    = \ & \sum^K_{k=1} V_1^{\pi_\ast} - V_1^{\pi_k} \\
    = \ & \sum^K_{k=1} V_1^{\pi_\ast} - \hat{V}_1^{\pi_k} + \hat{V}_1^{\pi_k}  - V_1^{\pi_k} \,.
\end{align*}

For any $h \in [1, H]$, by bellman equation and our update rule, we have
\begin{align*}
    & V_h^{\pi_\ast}(s) - \hat{V}_h^{\pi_k}(s) \\
    = \ & \langle Q_h^{\pi_\ast}(s, \cdot) , \pi_\ast(\cdot \mid s) \rangle - \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_k(\cdot \mid s) \rangle \\
    = \ & \langle Q_h^{\pi_\ast}(s, \cdot) -  \hat{Q}_h^{\pi_k}(s, \cdot), \pi_\ast(\cdot \mid s) \rangle + \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \\
    = \ & \mathbb{E}_{\pi_\ast} \left[ (r(s, a) - \hat{r}(s,a)) + (\sPsa (V_{h+1}^\ast)(s,a) -  \hPsa(\hVpn)(s,a)) - b_h^k(s,a)\right] \\
    & \ + \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \\
    = \ & \mathbb{E}_{\pi_\ast} \left[ (r(s, a) - \hat{r}(s,a)) +  (\sPsa(\hVpn)(s,a) -  \hPsa(\hVpn)(s,a))) - b_h^k(s,a)\right] \\
    & \ + \mathbb{E}_{\pi_\ast} \left[  \sPsa (V_{h+1}^\ast)(s,a) - \sPsa(\hVpn)(s,a)\right] + \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \,.
\end{align*}

By the design of our bonus function, with probability $ 1 - 2/ H$, we have
\begin{align*}
     (r(s, a) - \hat{r}(s,a)) + (\sPsa (V_{h+1}^\ast)(s,a) -  \hPsa(\hVpn)(s,a)) - b_h^k(s,a) \leq 0 \,.
\end{align*}

Notice that $\sPsa (V_{h+1}^\ast)(s,a) - \sPsa(\hVpn)(s,a) \leq \sup_{p\in \gP_h} p_h(\cdot \mid s,a) (V_{h+1}^\ast - \hVpn) $. Then, by recursion, we have 
\begin{align*}
    \sum^K_{k=1}V_1^{\pi_\ast}(s) - \hat{V}_1^{\pi_k}(s)
    \le \sum^K_{k=1} \sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \right] \,,
\end{align*}
where $q_h = \arg\max_{p\in \gP_h} p_h(\cdot \mid s,a) (V_{h+1}^\ast - \hVpn)$.

By the fundamental inequality of online mirror descent (\cite{orabona2019modern} Theorem 10.4), we have
%\dong{add expect}
\begin{align*}
    \sum^K_{k=1} \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \leq \frac{\log (A)}{\beta} + \frac{\beta}{2} \sum^K_{k=1} \sum_{a \in \gA} \pi_h^\ast (a \mid s) (\hat{Q}_h^{\pi_k}(s, a) )^2 \,.
\end{align*}
By the update rule, we have $\hat{Q}_h^{\pi_k}(s, a) \in [0, H]$, for all $h, k$. Then take $\beta = \sqrt{\frac{2 \log A}{H^2 K}}$ we have 
\begin{align*}
     \sum^K_{k=1}V_1^{\pi_\ast}(s) - \hat{V}_1^{\pi_k}(s) = \Tilde{O} \left(H^2\sqrt{K} \right)\,.
\end{align*}
{\color{blue} TODO: Need to create good events. }


\paragraph{Bounding the estimation error}

By the algorithm's update rule and the robust bellman equation, we have 
\begin{align*}
    (\hVp - \Vp )(s)
    = \ & \langle \hQp (s, \cdot) - \Qp (s, \cdot) , \pi_k(\cdot \mid s) \rangle \\
    = \ & \left\langle \hat{r}(s, \cdot) - r(s, \cdot)  + ( \hPsa(\hVpn)(s,\cdot) - \sPsa (\Vpn)(s,\cdot) ) + b_h^k(s,\cdot),  \pi_k(\cdot \mid s) \right\rangle  \,.
\end{align*}
By adding and subtracting a term $\sPsa (\hVpn)(s) $, we have 
\begin{align*}
    & \hPsa(\hVpn)(s,\cdot) - \sPsa (\Vpn)(s,\cdot) \\
    = \ & \hPsa(\hVpn)(s,\cdot)  - \sPsa (\hVpn)(s,a) + \sPsa (\hVpn)(s,a)  - \sPsa (\Vpn)(s,\cdot)\\
    \leq \ &   \hPsa (\hVpn)(s,\cdot) - \sPsa (\hVpn)(s,\cdot) + \arg\max_{P_h \in \gP_h}P_h(\cdot \mid s,a)( \hVpn - \Vpn) \,.
\end{align*}

Define $q_h = \arg\max_{P_h \in \gP_h} \limits P_h(\cdot \mid s,a)(\hVpn - \Vpn)$, $q = \{q_h\}$, we have
\begin{align*}
    & (\hVp - \Vp )(s) \\
    \leq \ & \mathbb{E}_{\pi_k}\left[ (r(s, a) - \hat{r}(s, a)) + \left( \hPsa(\hVpn)(s,a) - \sPsa (\hVpn)(s,a)  \right) + b_h^k(s,a) + q_h (\hVpn - \Vpn )(s,a) \right]\,.
\end{align*}

By doing a recursion with $q_h$ and noticing $V_{H+1}^{\pi_k} = \hat{V}_{H+1}^{\pi_k} = 0$, we have
\begin{align*}
    & (\hat{V}_1^{\pi_k} - V_1^{\pi_k})(s) \\
    \leq \ &\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ (r(s, a) - \hat{r}(s, a)) + \left( \hPsa(\hVpn)(s,a) -  \sPsa (\hVpn)(s,a) \right) + b_h^k(s,a)\right]\,.
\end{align*}

In the case of $(s,a)$-rectangular set, we have
\begin{align*}
    & \sPsa (\hVpn)(s,a) 
    = \  \inf_{P_h \in \gP_h(s,a)} \sum_{s^\prime} P_h(s^\prime \mid s,a) \hVpn(s^\prime) \\
     \text{subject to } & \sum_{s^\prime} | P_h(s^\prime \mid s,a) - P_h^o(s^\prime \mid s,a)| \leq \rho \,, \\
    &  \sum_{s^\prime} P_h(s^\prime \mid s,a) = 1 \,, \\
    &  P_h(\cdot \mid s,a) << P_h^o(\cdot \mid s,a)\,.
\end{align*}
{\color{blue} How do I align this?}

Define $\Tilde{P}_h(s^\prime \mid s, a) = \frac{ P_h(s^\prime \mid s,a) }{ P_h^o(s^\prime \mid s,a)}$, we can rewrite the above equation as
\begin{align*}
    & \sPsa (\hVpn)(s,a) 
    = \  \inf_{P_h \in \gP_h(s,a)} \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) \hVpn(s^\prime) \\
     \text{subject to } & \sum_{s^\prime} | \Tilde{P}_h(s^\prime \mid s,a)  - 1| P_h^o(s^\prime \mid s,a) \leq \rho \,, \\
    &  \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) = 1 \,, \\
    &  \Tilde{P}_h(s^\prime \mid s,a) \ge 0 \quad \forall s^\prime \in \gS\,.
\end{align*}

We can obtain the Lagrangian $L(\Tilde{P}_h, \eta, \lambda)$ with Lagrangian multiplier $\eta\in \mathbb{R}, \lambda\geq 0$,
\begin{align*}
    L(\Tilde{P}_h, \eta, \lambda) (s,a) 
    = \ & \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) \hVpn(s^\prime) + \lambda \left( \sum_{s^\prime} | \Tilde{P}_h(s^\prime \mid s,a)  - 1| P_h^o(s^\prime \mid s,a)  - \rho \right) \\
    & \ - \eta \left(\sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) - 1 \right) \,.
\end{align*}

Let $f(x) = |x - 1|$, then the convex conjugate of $f$, $f^\ast(y) = \sup_{x} \limits ( \langle x, y\rangle - f(x) )$. 
Using $f^\ast$, we can thus optimize over $\Tilde{P}_h$ and rewrite the Lagrangian over as 
\begin{align*}
    L(\eta, \lambda) (s,a) 
    = \ & \eta - \lambda \rho - \lambda \sum_{s^\prime}P_h^o(s^\prime \mid s,a) f^\ast \left(\frac{1}{\lambda} \left(\eta - \hVpn(s^\prime)\right) \right) \,.
\end{align*}
Notice that when $x \geq 0$, $f^\ast(y)$ has value $-1$ when $y \leq -1$, $f^\ast(y)=y$ when $y \in [-1, 1]$ and $f^\ast(y) = \infty$, when $y > 1$. Let $\Tilde{\eta} = \eta + \lambda$, then using the values of $f^\ast(y)$ and the equality $\max\left\{a,b\right\} = (a - b)_{+} + b$, we can rewrite the optimization problem as
\begin{align*}
    \sup_{\lambda \geq 0,  \Tilde{\eta} - \min_s \limits \hVpn(s) \leq 2 \lambda} \Tilde{\eta} - (\rho + 2) \lambda - \sum_{s^\prime}P_h^o(s^\prime \mid s,a) \left( \Tilde{\eta} - \hVpn(s^\prime)\right)_{+} \,.
\end{align*}

Optimize over $\lambda$, we can simplify the above problem into 
\begin{align*}
    \sup_{\Tilde{\eta}} \Tilde{\eta} - \frac{ (\Tilde{\eta} - \min_s \limits \hVpn(s))_{+}}{2}(\rho + 2) - \sum_{s^\prime}P_h^o(s^\prime \mid s,a) \left( \Tilde{\eta} - \hVpn(s^\prime)\right)_{+} \,.
\end{align*}
Define $g(\Tilde{\eta}, P_h^o)$ as 
\[
g(\Tilde{\eta}, P_h^o) = \sum_{s^\prime}P_h^o(s^\prime \mid s,a) \left( \Tilde{\eta} - \hVpn(s^\prime)\right)_{+}  - \Tilde{\eta} + \frac{ (\eta - \min_s\limits  \hVpn(s))_{+}}{2} (\rho + 2) \,.
\]
First notice that $g$ is a convex function. Moreover, notice that when $\Tilde{\eta} \leq 0$, $g(\Tilde{\eta}, P_h^o) = - \Tilde{\eta} \geq 0$. When $\Tilde{\eta} = 2 \rho + 2H$, $g(\Tilde{\eta}, P_h^o) \geq 0$. 
Thus it suffice to optimize $g(\Tilde{\eta}, P_h^o)$ within the range of $\Tilde{\eta} \in [0, 2 \rho + 2H]$.

We can thus rewrite 
\begin{align*}
    \hPsa(\hVpn)(s,a) - \sPsa (\hVpn)(s,a)  
    = \ & \inf_{\eta_1 \in [0, 2 \rho + 2H] } g(\eta_1, \hat{P}_h) - \inf_{\eta_2 \in [0, 2 \rho + 2H] }g(\eta_2, P_h^o)\\
    \leq \ & \sup_{\eta \in [0, 2\rho + 2H ]} | g(\eta, \hat{P}_h)  - g(\eta, P_h^o) |\,.
\end{align*}
With $\eta \in [0, 2\rho + 2H ]$ and by Holder's inequality, we have 
\begin{align*}
    | g(\eta, \hat{P}_h)  - g(\eta, P_h^o) |
    = \ & \left|  \sum_{s^\prime}\hat{P}_h(s^\prime \mid s,a) \left( \eta - \hVpn(s^\prime)\right)_{+}  - \sum_{s^\prime}P_h^o(s^\prime \mid s,a) \left( \eta - \hVpn(s^\prime)\right)_{+} \right|  \\
    \leq \ & \left\|\hat{P}_h(\cdot \mid s,a) -  P_h^o(\cdot \mid s,a)\right\|_1 \| \eta - \hVpn(s)\|_\infty \\ 
    \leq \ & (2 \rho + H) \left\|\hat{P}_h(\cdot \mid s,a) -  P_h^o(\cdot \mid s,a)\right\|_1 
\end{align*}

By Hoeffding's inequality and an union bound over all $s,a$, the following inequality holds with probability at least $1 - \delta$
\begin{align*}
    \left\|\hat{P}_h(\cdot \mid s,a) -  P_h^o(\cdot \mid s,a)\right\|_1 \leq \sqrt{\frac{4 S \log(3SAH^2K/ \delta)}{N_h^k(s,a)}} \,.
\end{align*}
{\color{blue} TODO: put this as a good event.}

To bound $\sup_{\eta\in [0, 2\rho + 2H ]} | g(\eta, \hat{P}_h)  - g(\eta, P_h^o) |$ with high probability, we first create an $\epsilon$-net $N_\epsilon(\eta)$ with $g$ over $\eta\in [0, 2\rho + 2H ]$ such that
\begin{align*}
    \sup_{\eta\in [0, 2\rho + 2H ]} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \leq \sup_{\eta\in N_\epsilon(\eta)} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| + 2 \epsilon \,.
\end{align*}
Taking an union bound over $N_\epsilon(\eta)$, we have 
\begin{align*}
    \sup_{\eta\in [0, 2\rho + 2H ]} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \leq (2 \rho + H)\sqrt{\frac{4 S \log(3SAH^2K | N_\epsilon(\eta)| / \delta)}{N_h^k(s,a)}} + 2 \epsilon \,.
\end{align*}

Notice that $g$ is a $\frac{6 + \rho}{2}$-Lipschitz function over $\eta\in [0, 2\rho + 2H ]$, thus we have $| N_\epsilon(\eta)| = O\left(\frac{6 + \rho}{2 \epsilon}\right)$. Hence, we have
\begin{align*}
    \sup_{\eta\in [0, 2\rho + 2H ]} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \leq  (2 \rho + H) \sqrt{\frac{4 S \log(3SAH^2K (6 + \rho)/2\epsilon \delta)}{N_h^k(s,a)}} + 2 \epsilon\,.
\end{align*}
Take $\epsilon = \frac{6 + \rho}{2 H\sqrt{K}}$, we have
\begin{align*}
    \sPsa (\hVpn)(s,a)  - \hPsa(\hVpn)(s,a)
    \leq \ & \sup_{\eta\in [0, 2\rho + 2H ]} |  g(\eta, \hat{P}_h)  - g(\eta, P_h^o)| \\
    \leq \ &  (2 \rho + H) \sqrt{\frac{4 S \log(3SAH^2K^{3/2}/ \delta)}{N_h^k(s,a)}} + \frac{6 + \rho}{H\sqrt{K}}\,.
\end{align*}

By Hoeffding's inequality and an union bound on all $(s,a)$, we also have the following with probability at least $1- \delta$
\begin{align*}
    |r(s,a) - \hat{r}(s,a)| \leq \sqrt{\frac{2 \log(3SAH^2K/ \delta)}{N_h^k(s,a)}}  \,.
\end{align*}

Thus, by setting $\delta^\prime = 2 \delta$, $\delta = 1/ H$, then with probability at least $1 - 2/ H$, we have
\begin{align*}
     \sum^K_{k=1}(\hat{V}_1^{\pi_k} - V_1^{\pi_k})(s) 
    \leq \ &\sum^K_{k=1}\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ 2 b_h^k(s,a)\right]\\
    \leq \ & \sqrt{K}(6 + \rho) + O \left( (\rho + H) \sqrt{S \log(SAHK^{3/2})} \right)\sum^K_{k=1}\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[\sqrt{\frac{1}{N_h^k(s,a)}} \right]\,.
\end{align*}

By Lemma 7.5 of RL theory book {\color{blue} add reference here}, 
we have 
\begin{align*}
    \sum^K_{k=1}\sum^H_{h=1} \sqrt{\frac{1}{N_h^k(s,a)}} \leq 2 H \sqrt{SAK} \,.
\end{align*}
Combining everything, with probability at least $1 - 2/ H$, we have
\begin{align*}
    \sum^K_{k=1}(\hat{V}_1^{\pi_k} - V_1^{\pi_k})(s)  = \Tilde{O} \left((\rho + H) HS\sqrt{AK} \right) \,.
\end{align*}


==> sketch.tex <==
\begin{proofsketch}
We start with decomposing the regret as follows,
    \begin{align*}
    \text{Regret}(K) 
    = \  \sum^K_{k=1} V_1^{\ast}(s) - V_1^{\pi_k}(s)
    = \  \sum^K_{k=1}\left(\hat{V}_1^{\pi_k} (s) - V_1^{\pi_k}(s)\right) + \sum^K_{k=1} \left(V_1^{\ast} (s)- \hat{V}_1^{\pi_k}(s) \right)\,.
    \end{align*}
    
    For the first term, for any $h \in [H]$, we can further decompose it as 
    \begin{align*}
    (\hVp - \Vp )(s)
    %= \ & \langle \hQp (s, \cdot) - \Qp (s, \cdot) , \pi_k(\cdot \mid s) \rangle \\
    = \ & \left\langle \hat{r}(s, \cdot) - r(s, \cdot)  + ( \hPsa(\hVpn)(s,\cdot) - \sPsa (\Vpn)(s,\cdot) ) + b_h^k(s,\cdot),  \pi_k(\cdot \mid s) \right\rangle  \,.
\end{align*}
    Under the convention of optimism, we should hope that the bonus function $b_h^k(s,a)$ ``covers'' the estimation errors of the reward and transition functions. That is $r(s, a) - \hat{r}(s,a)$ and $\sPsa(\hVpn)(s,a) -  \hPsa(\hVpn)(s,a)$ are both smaller than our choice of bonus function. We now show that this is indeed the case under our designed bonus function.
    
    The estimation error of the rewards can rather be straightforwardly upper bounded by Hoeffding's inequality and an union bound argument. In contrast, the estimation error of $\sPsa(\hVpn)(s,a) -  \hPsa(\hVpn)(s,a)$ cannot be controlled by direct applications of concentration inequalities due to the presence of the $\sigma$ operator. Therefore, we resort to a primal-dual argument to first simply the problem into a $1$-dimensional convex optimization problem, where the estimation error can be better quantified. Similar primal-dual techniques are also used in previous works for robust dynamic programming and robust RL \cite{iyengar2005robust,panaganti2022sample,yang2021towards}. (\dong{this part is very bad})
    
%    First note that in the case of $(s,a)$-rectangular set, we have
%\begin{align*}
%    & \sPsa (\hVpn)(s,a) 
%    = \  \inf_{P_h \in \gP_h(s,a)} \sum_{s^\prime} P_h(s^\prime \mid s,a) %\hVpn(s^\prime) \\
%     \text{subject to } & \sum_{s^\prime} | P_h(s^\prime \mid s,a) - P_h^o(s^\prime \mid s,a)| \leq \rho \,, \\
%    &  \sum_{s^\prime} P_h(s^\prime \mid s,a) = 1 \,, \\
%    &  P_h(\cdot \mid s,a) << P_h^o(\cdot \mid s,a)\,.
%\end{align*}
Through a change of variable with $\Tilde{P}_h(s^\prime \mid s, a) = \frac{ P_h(s^\prime \mid s,a) }{ P_h^o(s^\prime \mid s,a)}$, we can write the Lagrangian form of $\sPsa (\hVpn)(s,a)$ as
\begin{align*}
    L(\Tilde{P}_h, \eta, \lambda) (s,a) 
    = \ & \sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) \hVpn(s^\prime) + \lambda \left( \sum_{s^\prime} | \Tilde{P}_h(s^\prime \mid s,a)  - 1| P_h^o(s^\prime \mid s,a)  - \rho \right) \\
    & \ - \eta \left(\sum_{s^\prime} \Tilde{P}_h(s^\prime \mid s,a) P_h^o(s^\prime \mid s,a) - 1 \right) \,,
\end{align*}
where $\eta, \lambda$ are both Lagrangian multipliers. 
Under the characterization of $\ell_1$ distance, we can use the convex conjugate of $f(x) = |x - 1|$ to optimize out $\Tilde{P}$, resulting with 
\begin{align}\label{eq:reduced_sa}
    \sup_{\lambda \geq 0,  \eta - \min_s \limits \hVpn(s) \leq 2 \lambda} \eta - \rho \lambda - \sum_{s^\prime}P_h^o(s^\prime \mid s,a) \left( \eta - \hVpn(s^\prime)\right)_{+} \,.
\end{align}
Notice that now $\sPsa(\hVpn)(s,a) -  \hPsa(\hVpn)(s,a)$ is equivalent to the difference between the two solutions of equation \ref{eq:reduced_sa} with the $P_h^o$ and $\hat{P}_h^{o,k}$. Moreover, this difference in the $P_h^o$ only incurs a difference in the value of $\sum_{s^\prime}P_h^o(s^\prime \mid s,a) \left( \eta - \hVpn(s^\prime)\right)_{+}$, which we can use Hoeffding's inequality to control the difference if $\eta$ is bounded. Lastly, we investigate the range of possible optimal values of $\eta$ and use an $\epsilon$-net argument to account for the supremum.

By the optimism achieved by our bonus function, we have
\begin{align*}
     \sum^K_{k=1}(\hat{V}_1^{\pi_k} - V_1^{\pi_k})(s) 
    \leq \ \sum^K_{k=1}\sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ 2 b_h^k(s,a)\right]
    \leq \ O \left(H^2 S\sqrt{AK \log \left( SAH^2 K^{3/2} ( 1 + \rho) / \delta \right)} \right)\,.
\end{align*}


Then we consider the second term. For any $h \in [1, H]$, by bellman equation and our update rule, it can be decomposed as 
\begin{align*}
    & V_h^{\ast}(s) - \hat{V}_h^{\pi_k}(s) \\
    = \ & \mathbb{E}_{\pi_\ast} \left[ (r(s, a) - \hat{r}(s,a)) +  (\sPsa(\hVpn)(s,a) -  \hPsa(\hVpn)(s,a)) - b_h^k(s,a)\right] \\
    & \ + \mathbb{E}_{\pi_\ast} \left[  \sPsa (V_{h+1}^\ast)(s,a) - \sPsa(\hVpn)(s,a)\right] + \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \,.
\end{align*}

By the design of our bonus function and a recursion, we can obtain
\begin{align*}
    \sum^K_{k=1}V_1^{\ast}(s) - \hat{V}_1^{\pi_k}(s)
    \le \sum^K_{k=1} \sum^H_{h=1} \mathbb{E}_{\pi_k, \{q_h\}^H_{h=1}} \left[ \langle \hat{Q}_h^{\pi_k}(s, \cdot) , \pi_\ast(\cdot \mid s) - \pi_k(\cdot \mid s)  \rangle \right] \leq \Tilde{O} \left(H^2 \sqrt{K}\right) \,,
\end{align*}
where $q_h = \arg\max_{p\in \gP_h} p_h(\cdot \mid s,a) (V_{h+1}^\ast - \hVpn)$ and the last inequality is by standard results for online mirror descent.

Combining the two results yields the final regret upper bound.
\end{proofsketch}
